Introduction to Functional Classes in CS1

Students introduced to programming using a design-based approach and a functional programming language become familiar with first-class functions. They rarely, however, connect first-class functions to objects and object-oriented program design. This is a missed opportunity because students inevitably go on to courses using an object-oriented programming language. This article describes how students are introduced to objects within the setting of a design-based introduction to programming that uses a functional language. The methodology exposes students to interfaces, classes, objects, and polymorphic dispatch. Initial student feedback suggests that students benefit from the approach.

==> eptcsdata.tex <==
\providecommand{\firstpage}{114}
\providecommand{\publicationstatus}{P. Achten \& E. Machkasova  (Eds.): Trends in\\
Functional Programming in Education (TFPIE) 2021/22
\\
EPTCS 363, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.363.7}{10.4204/EPTCS.363.7}}
\pdfoutput=1

